Equivalence classes of augmentations and Morse complex sequences of Legendrian knots

Let L be a Legendrian knot in R^3 with the standard contact structure. In [10], a map was constructed from equivalence classes of Morse complex sequences for L, which are combinatorial objects motivated by generating families, to homotopy classes of augmentations of the Legendrian contact homology algebra of L. Moreover, this map was shown to be a surjection. We show that this correspondence is, in fact, a bijection. As a corollary, homotopic augmentations determine the same graded normal ruling of L and have isomorphic linearized contact homology groups. A second corollary states that the count of equivalence classes of Morse complex sequences of a Legendrian knot is a Legendrian isotopy invariant.

==> Sections/Preamble.tex <==
% This is the preamble of the document where Theorem-type environments are defined. Common shortcuts and document-specific notation are also defined here.
% Michael Brad Henry

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\makeatletter
\newtheorem*{rep@corollary}{\rep@title}
\newcommand{\newrepcorollary}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@corollary}}%
 {\end{rep@corollary}}}
\makeatother

% Theorems and such
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newreptheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newrepcorollary{corollary}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{case}{Case}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{property}{Property}
\newtheorem{step}{Step}
\newtheorem*{condition}{Condition}
\newtheorem{question}{Question}
\newtheorem{remark}[theorem]{Remark}

\theoremstyle{remark}
\newtheorem*{example}{Example}
\newtheorem*{note}{Note}


% Shortcut to ``blackboard bold'' and script letters
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\pp}{\ensuremath{\mathbb{P}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\alg}{\ensuremath{\mathcal{A}}}
\newcommand{\bbc}{\ensuremath{\mathcal{B}}}
\newcommand{\rrc}{\ensuremath{\mathcal{R}}}
\newcommand{\wwc}{\ensuremath{\mathcal{W}}}
\newcommand{\vvc}{\ensuremath{\mathcal{V}}}
\newcommand{\ttc}{\ensuremath{\mathcal{T}}}
\newcommand{\ssc}{\ensuremath{\mathcal{S}}}
\newcommand{\llc}{\ensuremath{\mathcal{L}}}
\newcommand{\kkc}{\ensuremath{\mathcal{K}}}
\newcommand{\nnc}{\ensuremath{\mathcal{N}}}
\newcommand{\xxc}{\ensuremath{\mathcal{X}}}
\newcommand{\mmc}{\ensuremath{\mathcal{M}}}

\newcommand{\cc}{\ensuremath{\mathbb{C}}}

\newcommand{\df}{\ensuremath{\partial}}
\newcommand{\aug}{\ensuremath{\epsilon}}
\newcommand{\MCS}{\ensuremath{\mathcal{C}}}
\newcommand{\Leg}{\ensuremath{L}}
\newcommand{\ruling}{\ensuremath{\rho}}
\newcommand{\front}{\ensuremath{D}}
\newcommand{\ring}{\ensuremath{R}}
\newcommand{\field}{\ensuremath{\mathbb{F}}}
\newcommand{\Maslov}{\ensuremath{\mu}}
\newcommand{\Zm}{\ensuremath{\mathbb{Z} / m \mathbb{Z}}}
\newcommand{\rank}{\ensuremath{\mbox{rank }}}

%Brad:  Some of thesee notations may look nicer if you use $\mathit{Aug}_m(D;\F)$ which will typeset slightly differently than $Aug_m(D;\F)$.  In the latter the Aug part is designed to appear as a product of A u and g.

%Notation agreed upon during Dan's visit to Siena
%
%Legendrian knot/link: $L$
%
%Normal ruling: $\rho$
%
%Grading: $m$
%
%Field: $\mathbb{F}$ (or shortcut $\F$)
%
%A prime number: $p$ 
%
%Front diagram of $L$: $D$
%
%CE-DGA of $D$: $(\mathcal{A}(D), \partial)$
%
%The set of $m$-graded augmentations to $F$ of $(\mathcal{A}(D), \partial)$:  $\overline{Aug}_m(D;\F)$
%
%Normalized $m$-graded augmentation invariant: $Aug_m(D;\F)$
%
%The set of $A$-form $m$-graded MCSs over $\F$: $MCS_m^{A}(D;\F)$
%
%The set of $SR$-form $m$-graded MCSs over $\F$: $MCS_m^{SR}(D;\F)$


%Extra and possibly unnecessary code of unknown origin. I am hesistant to remove it until I am sure it is unneeded.

% Adrian's magic label command
\newcommand{\mylabel}[1]{\label{#1}
%Comment this part out to remove the label boxes
%\fbox{\upshape \tiny {#1}}
}

\providecommand{\MR}{\relax\ifhmode\unskip\space\fi MR }
% \MRhref is called by the amsart/book/proc definition of \MR.
\providecommand{\MRhref}[2]{%
  \href{http://www.ams.org/mathscinet-getitem?mr=#1}{#2}
}
\providecommand{\href}[2]{#2}
